Can Machines Resonate with Humans? Evaluating the Emotional and Empathic Comprehension of LMs

Empathy plays a pivotal role in fostering prosocial behavior, often triggered by the sharing of personal experiences through narratives. However, modeling empathy using NLP approaches remains challenging due to its deep interconnection with human interaction dynamics. Previous approaches, which involve fine-tuning language models (LMs) on human-annotated empathic datasets, have had limited success. In our pursuit of improving empathy understanding in LMs, we propose several strategies, including contrastive learning with masked LMs and supervised fine-tuning with large language models. While these methods show improvements over previous methods, the overall results remain unsatisfactory. To better understand this trend, we performed an analysis which reveals a low agreement among annotators. This lack of consensus hinders training and highlights the subjective nature of the task. We also explore the cultural impact on annotations. To study this, we meticulously collected story pairs in Urdu language and find that subjectivity in interpreting empathy among annotators appears to be independent of cultural background. Our systematic exploration of LMs' understanding of empathy reveals substantial opportunities for further investigation in both task formulation and modeling.

==> Assets/arslan_dataset.tex <==
% \section{Analysis}
\section{Collective Human Opinions}
\label{sec:datasetanalysis}
% We speculate that high human disagreement exists in empathic similarity labeling due to extreme subjectivity. write more 
To analyze the subjectivity in empathic similarity labeling, we first collect eight annotations for each English story pairs, and then investigate the impact of the language/culture on the empathy labeling by collecting and annotating Urdu story pairs.

\begin{table*}[t!]
    \centering
    \resizebox{\textwidth}{!}{
    \begin{tabular}{@{}lcccccccccccccccccccc@{}}
    \toprule
    %\multicolumn{1}{l|}{\textbf{Dataset Labels$\rightarrow$}} & \multicolumn{10}{c|}{\textbf{Development Set}} & \multicolumn{10}{c}{\textbf{Test Set}} \\
    \multicolumn{1}{l|}{\textbf{IAA Metric$\downarrow$}} & \textbf{S\_eve} & \textbf{S\_emo} & \textbf{S\_mor} & \textbf{S\_emp} & \textbf{F\_eve} & \textbf{F\_emo} & \textbf{F\_mor} & \textbf{F\_emp} & \textbf{Comb\_eve} & \multicolumn{1}{c|}{\textbf{Comb\_emo}} & \textbf{S\_eve} & \textbf{S\_emo} & \textbf{S\_mor} & \textbf{S\_emp} & \textbf{F\_eve} & \textbf{F\_emo} & \textbf{F\_mor} & \textbf{F\_emp} & \textbf{Comb\_eve} & \textbf{Comb\_emo} \\ 
    \midrule
    \multicolumn{10}{c}{\texttt{All annotators - 8}} & \multicolumn{10}{c}{Chinese / English Speakers (friends- 2)}\\ 
    \midrule
    \multicolumn{1}{l|}{\textbf{Pearson}} & 0.421 & 0.078 & 0.189 & 0.191 & 0.442 & 0.098 & 0.110 & -0.015 & 0.176  & \multicolumn{1}{c|}{0.141} & 0.735 & 0.322 & 0.192 & 0.148 & \textbf{0.848} & 0.311 & -0.086 & -0.241 & -0.302 & -0.153 \\
    \multicolumn{1}{l|}{\textbf{Spearman}} & 0.395 & 0.063 & 0.187 & 0.190 & 0.438 & 0.088 & 0.138 & 0.004 & 0.158 &  \multicolumn{1}{c|}{0.129} & 0.701 & 0.252 & 0.143 & 0.090 & \textbf{0.868} & 0.313 & -0.109 & -0.108 & -0.437 & -0.183 \\
    \multicolumn{1}{l|}{\textbf{KA}}  & 0.349 & 0.059 & 0.168 & 0.114 & 0.398 & 0.092 & 0.105 & 0.027 & 0.095 &   \multicolumn{1}{c|}{0.107} & 0.401 & 0.086 & 0.174 & -0.152 & 0.761 & 0.233 & -0.065 & -0.349 & -0.295 & -0.128
    \multicolumn{1}{l|}{\textbf{Cohen Kappa}} & 0.124 & -0.015 & 0.067 & 0.047 & 0.157 & -0.024 & 0.030 & 0.026 & 0.059  & \multicolumn{1}{c|}{0.049} & 0.143 & -0.045 & 0.024 & -0.013 & 0.359 & -0.053 & 0.067 & -0.039 & -0.364 & -0.061 \\
    \midrule

    \multicolumn{10}{c}{\texttt{English / Urdu Speakers (colleagues - 4)}} & \multicolumn{10}{c}{ English / Urdu speakers (sisters - 2)}\\ 
    \midrule
    \multicolumn{1}{l|}{\textbf{Pearson}} & 0.266 & 0.037 & 0.089 & 0.093 & 0.322 & -0.017 & 0.234 & -0.039 & 0.137 & \multicolumn{1}{c|}{0.071} & \textbf{0.836} & 0.728 & 0.698 & 0.771 & 0.683 & 0.697 & 0.278 & 0.504 & 0.625 & 0.238 \\
    \multicolumn{1}{l|}{\textbf{Spearma}} & 0.235 & 0.028 & 0.101 & 0.078 & 0.295 & -0.013 & 0.194 & -0.075 & 0.133 & \multicolumn{1}{c|}{0.065} & \textbf{0.754} & 0.686 & 0.695 & 0.787 & 0.523 & 0.577 & 0.301 & 0.455 & 0.577 & 0.221 \\
    \multicolumn{1}{l|}{\textbf{KA}} & 0.235 & 0.051 & 0.050 & 0.026 & 0.311 & -0.008 & 0.187 & 0.057 & 0.098 & \multicolumn{1}{c|}{0.030}  & 0.724 & 0.476 & 0.709 & 0.773 & 0.659 & 0.560 & 0.273 & 0.486 & 0.317 & 0.195 \\
    \multicolumn{1}{l|}{\textbf{Cohen Kappa}} & 0.113 & 0.053 & -0.030 & 0.007 & 0.114 & -0.040 & -0.006 & -0.070 & 0.015 &  \multicolumn{1}{c|}{-0.016} & \textbf{0.429} & 0.167 & 0.375 & 0.412 & \textbf{0.412} & -0.045 & 0.143 & 0.403 & 0.138 & -0.014 \\
    \bottomrule
    \end{tabular}%
    }
    \caption{Agreement scores for four groups. Summary and full story are abbreviated as S and F, Comb = S+F. and event, emotion, moral, and empathy are shortened as eve, emo, mor, and emp. KA refers to Krippendorff's Alpha.}
    \label{tab:agreement-score}
    % \vspace{-1em}
\end{table*}

\subsection{English Story Pair Annotation}
 % Annotator Disagreement on English Stories Pairs
We sample 10 stories pairs from the development sets of \empathicstories, and invite eight annotators to assign labels in three settings. 
%Their background information as the Table below. 

\paragraph{Annotation Setups}
\citet{shen-etal-2023-modeling} employed Amazon MTurk workers to annotate similarity scores based on the story summaries considering the heavy cognition load of understanding the full story. 
Upon performing qualitative analyses of both full stories and their summaries, we observed that summaries generated by GPT-3.5-turbo will dismiss many narratives presenting emotional changes (\textit{from depressed, to sad, finally turn to happy}), inner monologue (\textit{I feel alone after Mary left}) and details of other roles, only keeping the major events and tone of the full stories. 
While these details are very important to identify subtle feelings and affect the empathy.
Model predictions based on the full stories also significantly differ from those obtained via the summaries as shown in \secref{sec:exp}. %, as demonstrated in Table \ref{tab:lm-unsupervise-cosine}. 
% 
% To evaluate the subjectivity of the task using agreement scores
To this end, we collect annotations under three settings: 
\begin{compactitem} 
    \item \textbf{Continuous score on summary:} annotators assign similarity scores from event, emotion, moral and empathy by continuous value ranging from 1 to 4, based on the story summary.
    \item \textbf{Continuous score on full story:} same as above, while based on the full story pair.  % including 0.5 increments.
    \item \textbf{Discrete class-label on full story:} considering that continuous scores provide larger labeling space, it may exacerbate subjectivity and inner-annotator disagreements, annotators are asked to rate event and emotion similarity using class labels: very similar (V), moderately similar (M), and not similar (N). Here, we do not rate moral and empathy given they are too abstract concept to perceive and rate. 
\end{compactitem}
Based on the annotation results, we aim to measure and analyze the subjectivity of human opinions in different annotation setups, i.e., how the presentation of stories and the annotation scale influence human agreement.
% by comparing the agreement scores across different formats and scales.
Pearson and Spearman correlation, Krippendorff's Alpha, and Cohen Kappa (convert to discrete) are used to measure the inter-annotator agreement. We first calculate the agreement between any two annotators and then average.


\paragraph{Annotator Background}
Eight annotators are aged between 20 and 35 years, from diverse cultural and ethnic backgrounds, including two native Chinese speakers and 
six native Pakistan speakers, with a balanced gender distribution.
All annotators are proficient in English, some major in psychology with bachelor's degree and some are PhD and postdoc students in NLP. 
An annotation training was performed before the formal annotations, which instructed raters how to rate the similarity score and highlight the differences between event, emotion, moral and empathy (see annotation guidelines in \figref{fig:instruction}). 


\paragraph{Results and Analysis}
\tabref{tab:agreement-score} reveal three major findings.
% four aspects
Overall, the agreement for event is the highest, followed by emotion, empathy and the moral is the least over all metrics, groups and settings. This suggests that it is easier to annotators to reach consensus on more concrete aspects like event and emotion compared with more abstract concepts of moral and empathy.
% Specifically, the Pearson and Spearman correlations are moderate for event and emotion but drop significantly for moral and empathy. Krippendorff’s Alpha and Cohen Kappa further corroborate these trends, showing higher agreement for event and emotion compared to moral and empathy.

% four groups
The closer the relationship between two annotators, the higher agreement for more subtle aspects.
Two Chinese friends (one male, one female) exhibit the highest correlation on judging event similarity based on full story, but lower correlation on all other settings than the two Pakistan sisters.
They even achieve $r/\rho$ >0.7 for moral and empathy when the average is less than 0.2 based on story summary.
Four Pakistan colleagues show extremely low agreement with each other, correlations are around 0.3 for event and $r/\rho$<0.1 for other aspects, demonstrating the significant variability in how different individuals perceive and interpret the stories.
These findings to some extent indicate that individuals who have similar background and experiences tend to reach consensus in interpretations of the stories, particular for subtle and abstract concepts.
% This finding highlights the influence of personal relationships and shared cultural contexts on the perception of narratives. 

Moreover, varying agreement scores across different groups suggests that individual background and culture significantly influence how stories are perceived and annotated.
This subjectivity poses challenges for models to learn and replicate human-like judgements, especially for moral and empathy reasoning. 
The agreement of collective human opinions in similarity score annotations also presents the upper bound that a model can reach at best.
This explains the enhancement bottleneck of various modeling methods. 


% % Comparison of three annotation settings
Compared three settings, lower agreement is obtained when labeling with three classes than continuous scores.
Amongst, full story provides more details and leads to higher correlations than summary on average. 
This guides the setting of future annotations for empathy similarity task --- providing annotators with full stories and annotating concrete aspects like event and emotion using continuous labels.
Annotations of moral and empathy might become less meaningful given the extreme subjectivity leading to random labels.    

Given that all annotators are not English native speakers and not grown up from western cultures, bias might be introduced in labeling English stories pairs. We collect a set of Urdu stories and employ Urdu native speakers to annotate.
This aims to eliminate potential biases, and most importantly to investigate the impact of languages and culture on the empathy similarity labeling.

% Average agreement scores for all annotators are lower than those for separate groups, indicating significant variability in how different individuals perceive and interpret the stories. 
% The Pearson and Spearman correlation scores for event and emotion are particularly high, indicating a strong consensus among Chinese annotators on these aspects. However, the scores for moral and empathy are lower. 

% \textbf{Urdu Speakers:} Urdu speakers also show relatively high agreement scores, especially for event and emotion. Their Pearson and Spearman correlations suggest a good level of consensus. However, as with other groups, moral and empathy scores are lower, reflecting the inherent subjectivity in these aspects. 


% \textbf{Friends/Relatives:} This group shows the most correlation, particularly in event and emotion annotations. The high agreement among friends and relatives indicates that shared background and experiences may lead to more consistent interpretations of the stories. This finding highlights the influence of personal relationships and shared cultural contexts on the perception of narratives. The variability in agreement scores across different groups suggests that individual backgrounds and cultural contexts significantly influence how stories are perceived and annotated. 
%This subjectivity poses a challenge for language models (LMs) attempting to learn and replicate human-like empathy and moral reasoning. 

% Across all annotators, the average agreement scores for all annotators combined are lower than those for specific groups, indicating significant variability in how different individuals perceive and interpret the stories. 



\subsection{Urdu Dataset Construction}
% The findings in \tabref{tab:agreement-score} motivate us to create a new benchmark with stories containing richer emotional and empathy signals. 
Urdu is widely spoken in many south Asian countries, including Pakistan, India, Bangladesh, and Nepal. Roman Urdu/Hindi, which uses English alphabets to write Urdu or Hindi, is commonly used in these regions for communication, discussions, and sharing feelings on media platforms. Therefore, we collected stories written by Roman Urdu.
% The motivation of urdu dataset, the reason of Roman Urdu, 

\begin{table}[t!]
    \centering
    %\resizebox{\textwidth}{!}{
    \scalebox{0.72}{
    \begin{tabular}{@{}lcccc@{}}
    \toprule
    %\multicolumn{1}{l|}{\textbf{Dataset Labels$\rightarrow$}} & \multicolumn{10}{c|}{\textbf{Development Set}} & \multicolumn{10}{c}{\textbf{Test Set}} \\
    \multicolumn{1}{l|}{\textbf{IAA Metric$\downarrow$}} & \textbf{event} & \textbf{emotion} & \multicolumn{1}{c|}{\textbf{empathy}} & \textbf{overall} \\ 
    \midrule
    \multicolumn{1}{c}{\texttt{}}&\multicolumn{3}{c}{\texttt{All annotators (4)}} & \multicolumn{1}{|r}{GPT-4o}\\ 
    \midrule
    \multicolumn{1}{l|}{\textbf{Pearson}} & 0.307 & 0.380 &  \multicolumn{1}{c|}{0.421} & 0.425   \\
    \multicolumn{1}{l|}{\textbf{Spearman}} & 0.306 & 0.361 & \multicolumn{1}{c|}{0.392 } & 0.403 \\
    \multicolumn{1}{l|}{\textbf{KA}} & 0.214 & 0.316 & \multicolumn{1}{c|}{0.392} & 0.393 \\
    \multicolumn{1}{l|}{\textbf{Cohen Kappa}} & 0.132  & 0.168 & \multicolumn{1}{c|}{0.189} & 0.075 \\
       \bottomrule
    \end{tabular}%
    }
    \caption{Agreement scores of Urdu annotators for Roman Urdu dataset. On the right, the empathy scores of 4 annotators are averaged correspondingly and and compared with the GPT overall score.}
    \label{tab:urdu_agreement-score}
    % \vspace{-1em}
\end{table}

\begin{table}[t!]
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{@{}lccccccc@{}}
\toprule
\multicolumn{1}{l|}{\textbf{Gold Label$\downarrow$}} & \textbf{$r$} & \textbf{$\rho$} & \textbf{MSE}$\downarrow$ & \textbf{Acc} & \textbf{Prec} & \textbf{Recall} & \textbf{F1} \\ \midrule
\multicolumn{8}{c}{\texttt{OpenAI-text-embedding-3-large}} \\ \midrule
\multicolumn{1}{l|}{\textbf{Empathy}} & 0.486 & 0.527 & 1.610 & 0.296 & 0.609 & 0.562 & 0.289 \\
\multicolumn{1}{l|}{\textbf{Event}} & 0.539 & 0.548 & 1.040 & 0.399 & 0.651 & 0.564 & 0.372 \\
\multicolumn{1}{l|}{\textbf{Emotion}} & 0.493 & 0.529 & 1.600 & 0.292 & 0.607 & 0.562 & 0.286 \\ \midrule
\multicolumn{8}{c}{\texttt{Llama-3-8B}} \\ \midrule
\multicolumn{1}{l|}{\textbf{Empathy}} & 0.410 & 0.375 & 0.640 & 0.759 & 0.772 & 0.629 & 0.637 \\
\multicolumn{1}{l|}{\textbf{Event}} & 0.445 & 0.371 & 0.450 & 0.832 & 0.733 & 0.651 & 0.675 \\
\multicolumn{1}{l|}{\textbf{Emotion}} & 0.428 & 0.412 & 0.480 & 0.808 & 0.680 & 0.615 & 0.632 \\ \midrule
\multicolumn{8}{c}{\texttt{GPT-4o}} \\ \midrule
\multicolumn{1}{l|}{\textbf{Empathy}} & 0.715 & 0.725 & 0.330 & 0.797 & 0.762 & 0.757 & 0.759 \\
\multicolumn{1}{l|}{\textbf{Event}} & 0.772 & 0.762 & 0.310 & 0.842 & 0.760 & 0.848 & 0.786 \\
\multicolumn{1}{l|}{\textbf{Emotion}} & 0.774 & 0.774 & 0.310 & 0.818 & 0.732 & 0.807 & 0.754 \\ \bottomrule
\end{tabular}%
}
\caption{\textbf{Performance on Urdu dataset} over three types of gold similarity scores: \textbf{empathy}, \textbf{event}, and \textbf{emotion} using \textbf{cosine similarity($v_a$, $v_b$) with OpenAI embedding and zero-shot LLMs. Cosine similarity is normalized to the scale 1-4 by $\times$4. Classification gold labels are binned by $\text{score} > 2.5$.}}
\label{tab:urdu-llm-cosine}
\end{table}


\paragraph{Synthetic Story Pairs Generation}
After manually checking the quality of stories generated by GPT-4o,\footnote{We assess whether they are emotion-rich stories matching local culture.} we collect 300 story pairs by instructing GPT-4o to generate story pairs with varying similarity given a diverse range of domains and topics (see prompts in \figref{fig:urdustoryprompt}). 
Each pair consists of theme, content of two stories, an overall similarity score \textit{s} in [1,4], and a brief reason explaining why they are score as \textit{s}.  
 

% To synthetically generate pairs of stories for the Urdu dataset, we designed a prompt that creates around 300 pairs of stories in a balanced manner using the GPT-4o API. The themes mentioned in \citet{shen-etal-2023-modeling} were used in the prompts to maintain diversity and vocabulary balance in the stories. Additionally, we obtained overall similarity scores from GPT-4o for each pair of stories for later comparison with human annotations.
% The prompt, the balance we maintain in stories. the qualitiy

\paragraph{Human Annotations}
Four Urdu native speakers are employed to annotate similarity scores for event, emotion and empathy, ranging from 1 to 4 with increments of 0.5, in which moral is excluded due to the high ambiguity.
IAA among the four annotators are presented in \tabref{tab:urdu_agreement-score}. The last column \textit{overall} represents the agreement between the averaged empathy scores of the four annotators with the similarity score \textit{s} provided by GPT-4o in story generation. 
% We prepared 292 pairs of stories on diverse topics and themes for annotation. 
% The task was assigned to four human annotators with clear, example-containing instructions. Annotation scores were collected for Event, Emotion, and Empathy, while Moral was excluded due to its lowest correlation and highest ambiguity as found in Table \ref{tab:agreement-score}. The agreement scores for Event, Emotion, and Empathy among the four annotators are provided in Table \ref{tab:urdu_agreement-score}. The overall score represents the agreement between the average empathy scores of the four annotators and the overall similarity score from GPT-4o. 


\paragraph{LLM Estimations}

% \begin{table*}[tbh!]
%     \centering
%     \resizebox{\textwidth}{!}{
%     \begin{tabular}{@{}lcccccccccccccc@{}}
%     \toprule
%     \multicolumn{1}{l|}{\textbf{Model $\rightarrow$}} & \multicolumn{7}{c|}{\textbf{OpenAI-text-embedding-3-large}} & \multicolumn{7}{c}{\textbf{Llama 3}} \\
%     \multicolumn{1}{l|}{\textbf{Gold Label$\downarrow$}} & \textbf{$r$} & \textbf{$\rho$} & \textbf{MSE}$\downarrow$ & \textbf{Acc} & \textbf{Prec} & \textbf{Recall} & \multicolumn{1}{c|}{\textbf{F1-macro}} & \textbf{$r$} & \textbf{$\rho$} & \textbf{MSE}$\downarrow$ & \textbf{Acc} & \textbf{Prec} & \textbf{Recall} & \textbf{F1-macro} \\ 
%     \midrule
%     % \multicolumn{1}{c}{} & \multicolumn{7}{c}{\texttt{OpenAI-text-embedding-3-large} } & \multicolumn{7}{c}{\texttt{Llama 3} } \\ 
%     %\midrule
%     \multicolumn{1}{l|}{\textbf{Empathy}} & 0.486 & 0.527 & 1.610 & 0.296 & 0.609 & 0.562 & 0.289 & & & & & & & \\
%     \multicolumn{1}{l|}{\textbf{Event}} & 0.539 & 0.548 & 1.040 & 0.399 & 0.651 & 0.564 & 0.372 & & & & & & & \\
%     \multicolumn{1}{l|}{\textbf{Emotion}} & 0.493 & 0.529 & 1.600 & 0.292 & 0.607 & 0.562 & 0.286 & & & & & & & \\ \bottomrule
%     \end{tabular}%
%     }
%     \caption{\textbf{Cosine similarity($v_a$, $v_b$) across two sentence embedding models at Urdu dataset.} Results on three type of gold similarity scores: \textbf{empathy}, \textbf{event}, and \textbf{emotion} based. Cosine similarity is normalized to the scale 1-4 by $\times$4. Classification gold labels are binned by $\text{score} > 2.5$.}
%     \label{tab:urdu-llm-cosine}
% \end{table*}


% \paragraph{Discussion}


==> Assets/arslan_intro.tex <==
\section{Introduction}

In the rapidly evolving landscape of Natural Language Processing (NLP), understanding human emotions has become increasingly crucial. 
%With the advent of the Internet and the widespread use of social media, 
Individuals now share and express their thoughts, feelings, and experiences online more than ever before \cite{Sharma2022HumanAICE}. The ability of Large Language Models (LLMs) \cite{chang2024survey} to understand emotions in online interactions is essential as it enables more effective and empathetic human-computer interactions by responding appropriately to the emotional states of users. Emotional awareness is foundational to empathy, which is the cornerstone of building strong connections with others \cite{lin-etal-2023-ncuee}. 

Empathy fosters emotional resilience by allowing us to understand and share in the experiences of those around us. This, in turn, encourages prosocial actions, contributing positively to the world~\cite{Buecker2021IsLI}. The motivation behind studying empathic similarity is driven by the increasing recognition of empathy as a critical, yet underleveraged, component of interpersonal communication and connection \cite{Berridge2023CompanionRT}. 
%This is particularly important in applications such as virtual assistants, customer service bots, and mental health support systems, where understanding user emotions can significantly enhance the quality of interaction and user satisfaction. 
% Shen et al. (2023) proposed a novel approach to measuring empathic similarity between narratives. They defined it as the degree to which two personal stories resonate with each other across four aspects: events, emotions, morals, and the level of empathy evoked. This approach aimed to capture the shared emotional core of experiences.
\citet{shen-etal-2023-modeling} formulated the task EmpathicStories to assess the similarity between two narratives describing personal experiences from four aspects including event, emotion, moral and empathy. %The goal is to understand the story and assess how similar feelings are shared between the two stories.
However, fine-tuning LMs and prompting Large Language Models (LLMs) in their study resulted in low correlation with human judgments of empathic similarity.
% We hypothesize that the observed limitations arise from the fact that the models used were primarily trained for semantic similarity tasks, rather than being designed to capture empathy. Semantic similarity focuses on understanding the meanings of words and their relationships, yet it struggles to reason about the complex social and emotional dynamics present in human narratives \cite{Reimers2019SentenceBERTSE}. Consequently, while these models excel in tasks involving lexical and contextual similarities, they lack the nuanced comprehension needed to evaluate and reflect the emotional depth and empathy conveyed in human storytelling.
% After performing the extensive 

Our error analysis of the approaches by \citet{shen-etal-2023-modeling} reveals that the model struggles to identify correlations in the similar pairs of stories, while effectively recognizing dissimilar pairs. As shown in \secref{sec:casestudy}. The error rate increases with higher similarity between pairs. This suggests that the nuanced patterns and relationships in similar pairs are not effectively captured by semantically-oriented language models.  Semantic similarity focuses on understanding the meanings of words and their relationships, yet it struggles to reason about the complex social and emotional dynamics present in human narratives \cite{Reimers2019SentenceBERTSE}.   \par
We fine-tuned several LMs including MPNet \cite{song2020mpnet} Roberta \cite{Liu2019RoBERTaAR} (base, large), Deberta \cite{he2020deberta}(small, large), using a range of loss functions such as ContrastiveLoss, AnglELoss, CosineSimilarityLoss, CoSENTLoss, AnglELoss. %The experimental results in Table \ref{tab:lm-finetuning} show that the performance of these models on the Pearson and Spearman metrics does not improving beyond a certain threshold. 
Though we achieved around 5\% improvement in the Pearson, Spearman and Precision but these metrics does not improve beyond a certain threshold. We also explored the integration of Chain-of-Thought (CoT) reasoning and fine-tuning LLMs on the EmpathicStories dataset. For zero-shot settings of summaries, LLaMa-3 (70B) and GPT-4o showed good performance on Pearson and Spearman metrics for the event only. However, the three paradigms of supervised fine-tuning (SFT) of LLaMa-3-8B did not achieve satisfactory correlation scores for any of the gold labels.

This led us to hypothesize that language models struggle to learn and correlate human-annotated gold labels due to their subjective nature. To investigate this, we randomly selected 10 pairs of stories from the development set of the EmpathicStories dataset. These pairs were annotated by six different annotators from diverse demographics for Event, Emotion, Moral and Empathy similarity. Interestingly, the agreement scores among the annotators provided valuable insights. Overall agreement was low specifically for Moral, confirming the subjectivity of the task. On contrary, the highest agreement scores were observed among annotators from similar backgrounds. 



% While there are many ways to express empathy, they \cite{shen-etal-2023-modeling}  focus specifically on situational empathy, which is empathy that occurs in response to a social context, conveyed through text-based personal narratives. It transcends the mere act of listening, engaging the listener's ability to resonate emotionally with the storyteller \cite{Cho2019TheRO}. This concept taps into the fundamental human need for connection, validating our experiences and emotions in a world that often feels isolating \cite{Buecker2021IsLI}. 

% % \section{Motivation}
% . With the rise of loneliness, polarization, and social disconnection, there is an urgent need to harness technology not just for information exchange but for fostering genuine human connections. Empathic similarity offers a pathway to bridge emotional distances, enabling individuals to find common ground in their shared humanity, irrespective of their diverse backgrounds and life stories.

==> Assets/arslan_relatedwork.tex <==
\section{Related Work}
% Rewrite the related work, select the most relevant ones and organize them by subsetions. Maybe like:
\subsection{Emotion \& Empathy in LMs}
\citet{Sharma2020ACA} created a corpus EPITOME to facilitate a framework aimed at understanding empathy levels in online mental health conversations. Building on this, they later demonstrated \cite{Sharma2022HumanAICE} how Human-AI collaboration could enhance empathic communication in text-based mental health support, showing that peer supporters can effectively use AI-generated feedback to improve their responses to support seekers. This approach not only avoids over reliance on AI but also boosts the confidence of those providing support. \citet{Sharma2021TowardsFE} leveraged a Reinforcement Learning (RL) agent, which makes sentence-level edits to posts to increase empathy while maintaining conversation quality. The authors used the TalkLife dataset, a prominent online platform for mental health support, to train and evaluate system. 

Above work focused to generate the empathically rich conversation. However, in the recent study, West et al.  \cite{West2023TheGA} analyzed after controlled experiments that current AI models are far better than human in generating but fall short of human capabilities in a measure of understanding. Their findings support their hypothesis of that models’ generative capability may not be contingent upon understanding capability. We hypothesize that enhancing a model's empathy requires improving its ability to understand empathic nuances.

\citet{shen-etal-2023-modeling} proposed the task EmpathicStories to model the \textit{empathic similarity} in pair of stories (both narrates by different human) to enable the AI systems in understanding the empathic aspect at human level. The dataset contains scores (human-annotated) for three key features of the story: event, emotion, and moral, along with an overall empathy score. The authors reported the improved performance of semantic similarity models (SBERT, BART) after finetuning on proposed dataset. However, the absolute results achieved with LMs specifically on Pearson and Spearman are low. Our findings speculate that the reason is naive sentence embedding which consider semantic context only lead to lack in understanding the emotional and empathic signal.



%Inspired by the previous study which improve semantic embedding of sentences by downstreaming tasks of semantic textual similarity and natural language inference, we propose to improve empathic signal in embeddings by learning from empathic similarity task.  
% most previous work for Emotion and Empathy Understanding focus on emotion recognition and reasoning why it is this emotion by extracting reference snippets of text from the original text, for example... 
% However, Empathy similarity ... list the benefits of this dataset, (can find from the original paper) 

% However, very poor results obtained by the original work either based on BERT-like LMs or LLMs.
% We speculate that this is because naive sentence embeddings lack emotional and empathic signals.
% And naive LLM prompts does not fully empower LLMs' reasoning ability by CoT. %(see more in \secref{sec:casestudy}).
% Therefore, we propose to improve the empathy representation by ...


\subsection{Enhancing Semantic Embedding}
To enhance sentence embedding, \citet{Wu2021ESimCSEES} proposed ESimCSE which significantly improves sentence embeddings by %using contrastive learning techniques. They 
leveraging momentum contrast
method to increase the number of negative
pairs involved in the loss calculation, showing notable improvements across multiple semantic textual similarity benchmarks. \citet{hubert2024treat} improved the knowledge graph embeddings by integratign semantic awareness into traditional loss functions like pairwise hinge loss, binary cross-entropy loss, and logistic loss.
\citet{huang2024piccolo2} introduced Piccolo2, an embedding model that uses a multi-task hybrid loss training and a hard negative mining approach to better utilize textual data. Th study proposes a method for micro-gesture classification that incorporates both skeletal and semantic embedding loss functions. The approach enhances the model's performance by combining these losses, resulting in significant improvements in action classification tasks. 
% How people improved semantic sentence embedding by different loss function and methods.
% list methods and papers for losses we used in experiments.

% In this section, we aim to improve the empathy features in the embeddings, so we...


\subsection{LLM CoT and Fine-tuning}
Simplistic LLM prompts for EmpathicStories in \cite{shen-etal-2023-modeling} failed to fully leverage LLMs' reasoning capabilities. Recent advancements in few-shot and instruction prompting techniques include Chain-of-Thought prompting (CoT) \cite{wei2022chain}, Least-to-Most prompting \cite{zhou2022least}, and search-based approaches like Tree-of-Thought (ToT) \cite{yao2024tree}, and Graph-of-Thought \cite{besta2024graph}. AI systems still struggle to accurately recognize human emotions during conversations. Conversation models with large capacities, trained on unfiltered internet dialogues, often fail to exhibit empathy effectively \cite{shen2024empathicstories++}. It is highly important for LLMs to accurately comprehend user situations and craft responses that are not only contextually appropriate but also grounded in cognitive insights, linguistic patterns, and emotional context \cite{West2023TheGA, Zhou2023HowFA}. \citet{Luo2023CritiqueAO} examined the critique capabilities of LLMs, suggests that while these models can generate critique, their understanding of nuanced human emotions remains limited, reinforcing the need for further advancements in empathy understanding. \citet{Xue2023PACITUT} improved the instruction-following capabilities of LLMs by encouraging deep thinking about examples rather than just observing them. 

% YX: maybe we can say recent work \citet{shen-etal-2023-modeling} collect a dataset ... and propose .., However, describe their weaknesses.
% To this end, we .... (our plan)
%To foster deeper human connections, researchers have delved into the concept of empathic similarity \cite{shen-etal-2023-modeling}, focusing on the ability to understand and share another person's feelings through their narrative experiences. The authors have established a task and framework dedicated to measuring empathic resonance within personal narratives, enabling models to discern and learn the underlying reasons for similarities between pairs of stories.  



==> Assets/exp.tex <==
dev
Counter({3: 68, 2: 26, 4: 6})
\begin{tabular}{lrrrrrrr|rrrrrrr}
\toprule
 & \multicolumn{7}{|c}{\textbf{Development Set}} & \multicolumn{7}{|c}{\textbf{Test Set}} & 
 & Pearson & Spearman & MSE & accuracy & precision & recall & F1 \\
\midrule
empathy & 0.291 & 0.305 & 0.680 & 0.490 & 0.281 & 0.319 & 0.275 & 0.229 & 0.214 & 0.640 & 0.470 & 0.342 & 0.288 & 0.253 \\
event & 0.331 & 0.324 & 1.330 & 0.220 & 0.166 & 0.394 & 0.203 & 0.244 & 0.238 & 1.130 & 0.265 & 0.422 & 0.326 & 0.179 \\
emotion & 0.249 & 0.250 & 0.910 & 0.330 & 0.237 & 0.312 & 0.230 & 0.197 & 0.200 & 0.760 & 0.435 & 0.350 & 0.294 & 0.248\\
moral & 0.218 & 0.216 & 1.000 & 0.320 & 0.213 & 0.304 & 0.200 & 0.210 & 0.212 & 0.820 & 0.408 & 0.437 & 0.293 & 0.239 \\
\bottomrule
\end{tabular}


test-gold label by int()
\begin{tabular}{lrrrrrrr}
\toprule
 & Pearson & Spearman & MSE & accuracy & precision & recall & F1 \\
\midrule
empathy & 0.229 & 0.214 & 0.640 & 0.470 & 0.342 & 0.288 & 0.253 \\
event & 0.244 & 0.238 & 1.130 & 0.265 & 0.422 & 0.326 & 0.179 \\
emotion & 0.197 & 0.200 & 0.760 & 0.435 & 0.350 & 0.294 & 0.248 \\
moral & 0.210 & 0.212 & 0.820 & 0.408 & 0.437 & 0.293 & 0.239 \\
\bottomrule
\end{tabular}

test-gold label by >0.5 +1
\begin{tabular}{lrrrrrrr}
\toprule
 & Pearson & Spearman & MSE & accuracy & precision & recall & F1 \\
\midrule
empathy & 0.229 & 0.214 & 0.640 & 0.462 & 0.413 & 0.305 & 0.284 \\
event & 0.244 & 0.238 & 1.130 & 0.382 & 0.373 & 0.299 & 0.243 \\
emotion & 0.197 & 0.200 & 0.760 & 0.462 & 0.404 & 0.302 & 0.277 \\
moral & 0.210 & 0.212 & 0.820 & 0.435 & 0.377 & 0.285 & 0.254 \\
\bottomrule
\end{tabular}

test-gold label by original paper binning into 0/1
\begin{tabular}{lrrrrrrr}
\toprule
 & Pearson & Spearman & MSE & accuracy & precision & recall & F1 \\
\midrule
empathy & 0.229 & 0.214 & 0.640 & 0.572 & 0.628 & 0.564 & 0.506 \\
event & 0.244 & 0.238 & 1.130 & 0.368 & 0.616 & 0.580 & 0.363 \\
emotion & 0.197 & 0.200 & 0.760 & 0.532 & 0.626 & 0.563 & 0.482 \\
moral & 0.210 & 0.212 & 0.820 & 0.498 & 0.642 & 0.573 & 0.463 \\
\bottomrule
\end{tabular}

\subsection{Openai Embeddings Cosine similarity}
dev set: cosine similarity of openai embeddings: text-embedding-3-large
\begin{tabular}{lrrrrrrr}
\toprule
 & Pearson & Spearman & MSE & accuracy & precision & recall & F1 \\
\midrule
empathy & 0.335 & 0.315 & 4.790 & 0.620 & 0.310 & 0.500 & 0.383 \\
event & 0.437 & 0.411 & 2.900 & 0.830 & 0.415 & 0.500 & 0.454 \\
emotion & 0.394 & 0.350 & 4.400 & 0.710 & 0.355 & 0.500 & 0.415 \\
moral & 0.359 & 0.309 & 3.940 & 0.790 & 0.395 & 0.500 & 0.441 \\
\bottomrule
\end{tabular}

test set: cosine similarity of openai embeddings: text-embedding-3-large
\begin{tabular}{lrrrrrrr}
\toprule
 & Pearson & Spearman & MSE & accuracy & precision & recall & F1 \\
\midrule
empathy & 0.336 & 0.329 & 5.630 & 0.487 & 0.244 & 0.500 & 0.328 \\
event & 0.485 & 0.465 & 3.430 & 0.767 & 0.384 & 0.500 & 0.434 \\
emotion & 0.392 & 0.388 & 5.170 & 0.542 & 0.271 & 0.500 & 0.352 \\
moral & 0.366 & 0.356 & 4.860 & 0.603 & 0.301 & 0.500 & 0.376 \\
\bottomrule
\end{tabular}



\subsection{Llama3-70B result with different prompt/story type on two splits}

\begin{tabular}{lllllrrrrrrrrrrrr}
\toprule
 & model & split & prompt & story & F1-mean & F1-reverse & F1-standard & Pearson-mean & Pearson-reverse & Pearson-standard & Spearman-mean & Spearman-reverse & Spearman-standard & accuracy-mean & accuracy-reverse & accuracy-standard \\
\midrule
0 & Llama3-70B & dev & optimized & full & 0.42 & 0.49 & 0.56 & 0.26 & 0.18 & 0.25 & 0.28 & 0.17 & 0.25 & 0.46 & 0.50 & 0.57 \\
1 & Llama3-70B & dev & optimized & summary & 0.70 & 0.71 & 0.73 & 0.45 & 0.39 & 0.40 & 0.46 & 0.40 & 0.42 & 0.70 & 0.72 & 0.74 \\
4 & Llama3-70B & dev & optimized_brief & full & 0.66 & 0.66 & 0.61 & 0.26 & 0.27 & 0.19 & 0.27 & 0.29 & 0.19 & 0.70 & 0.71 & 0.68 \\
5 & Llama3-70B & dev & optimized_brief & summary & 0.49 & 0.46 & 0.46 & 0.46 & 0.47 & 0.36 & 0.45 & 0.47 & 0.34 & 0.66 & 0.65 & 0.65 \\
8 & Llama3-70B & dev & original & full & 0.27 & 0.27 & 0.35 & 0.09 & 0.03 & 0.10 & 0.09 & 0.03 & 0.12 & 0.37 & 0.36 & 0.42 \\
9 & Llama3-70B & dev & original & summary & 0.45 & 0.48 & 0.53 & 0.22 & 0.18 & 0.22 & 0.23 & 0.18 & 0.23 & 0.48 & 0.50 & 0.54 \\
12 & Llama3-70B & dev & original_brief & full & 0.69 & 0.68 & 0.73 & 0.37 & 0.33 & 0.33 & 0.39 & 0.35 & 0.38 & 0.69 & 0.69 & 0.74 \\
13 & Llama3-70B & dev & original_brief & summary & 0.68 & 0.61 & 0.70 & 0.36 & 0.29 & 0.36 & 0.38 & 0.29 & 0.38 & 0.71 & 0.68 & 0.74 \\
2 & Llama3-70B & test & optimized & full & 0.44 & 0.48 & 0.51 & 0.30 & 0.22 & 0.30 & 0.29 & 0.21 & 0.29 & 0.55 & 0.56 & 0.58 \\
3 & Llama3-70B & test & optimized & summary & 0.61 & 0.62 & 0.65 & 0.41 & 0.30 & 0.40 & 0.40 & 0.30 & 0.39 & 0.64 & 0.62 & 0.65 \\
6 & Llama3-70B & test & optimized_brief & full & 0.64 & 0.63 & 0.61 & 0.38 & 0.35 & 0.33 & 0.38 & 0.35 & 0.32 & 0.64 & 0.64 & 0.61 \\
7 & Llama3-70B & test & optimized_brief & summary & 0.43 & 0.40 & 0.41 & 0.41 & 0.34 & 0.39 & 0.41 & 0.34 & 0.38 & 0.54 & 0.53 & 0.53 \\
10 & Llama3-70B & test & original & full & 0.35 & 0.36 & 0.41 & 0.27 & 0.18 & 0.24 & 0.27 & 0.17 & 0.24 & 0.52 & 0.52 & 0.55 \\
11 & Llama3-70B & test & original & summary & 0.39 & 0.43 & 0.44 & 0.19 & 0.12 & 0.20 & 0.20 & 0.12 & 0.18 & 0.53 & 0.54 & 0.54 \\
14 & Llama3-70B & test & original_brief & full & 0.59 & 0.63 & 0.62 & 0.34 & 0.29 & 0.31 & 0.35 & 0.30 & 0.31 & 0.61 & 0.64 & 0.62 \\
15 & Llama3-70B & test & original_brief & summary & 0.62 & 0.59 & 0.60 & 0.31 & 0.26 & 0.29 & 0.31 & 0.26 & 0.30 & 0.62 & 0.60 & 0.62 \\
\bottomrule
\end{tabular}


\subsection{Llama3-8B-Instruct SFT results}
\subsubsection{Using Summary and empathy score only}
\paragraph{Dev}
\begin{tabular}{lrrrr}
\toprule
 & precision & recall & f1-score & support \\
\midrule
0 & 0.887 & 0.797 & 0.840 & 69.000 \\
1 & 0.632 & 0.774 & 0.696 & 31.000 \\
accuracy & 0.790 & 0.790 & 0.790 & 0.790 \\
macro avg & 0.759 & 0.786 & 0.768 & 100.000 \\
weighted avg & 0.808 & 0.790 & 0.795 & 100.000 \\
\bottomrule
\end{tabular}


\begin{tabular}{lrr}
\toprule
 & Spearman & Pearson \\
\midrule
0 & 0.470 & 0.476 \\
\bottomrule
\end{tabular}

\paragraph{Test}
\begin{tabular}{lrrrr}
\toprule
 & precision & recall & f1-score & support \\
\midrule
0 & 0.662 & 0.578 & 0.617 & 223.000 \\
1 & 0.541 & 0.627 & 0.581 & 177.000 \\
accuracy & 0.600 & 0.600 & 0.600 & 0.600 \\
macro avg & 0.602 & 0.603 & 0.599 & 400.000 \\
weighted avg & 0.608 & 0.600 & 0.601 & 400.000 \\
\bottomrule
\end{tabular}

\begin{tabular}{lrr}
\toprule
 & Spearman & Pearson \\
\midrule
0 & 0.307 & 0.320 \\
\bottomrule
\end{tabular}


\subsubsection{Using Full story and empathy score only}
\paragraph{Dev}
\begin{tabular}{lrrrr}
\toprule
 & precision & recall & f1-score & support \\
\midrule
0 & 0.806 & 0.725 & 0.763 & 69.000 \\
1 & 0.500 & 0.613 & 0.551 & 31.000 \\
accuracy & 0.690 & 0.690 & 0.690 & 0.690 \\
macro avg & 0.653 & 0.669 & 0.657 & 100.000 \\
weighted avg & 0.711 & 0.690 & 0.697 & 100.000 \\
\bottomrule
\end{tabular}

\begin{tabular}{lrr}
\toprule
 & Spearman & Pearson \\
\midrule
0 & 0.229 & 0.244 \\
\bottomrule
\end{tabular}



\paragraph{Test}

\begin{tabular}{lrrrr}
\toprule
 & precision & recall & f1-score & support \\
\midrule
0 & 0.708 & 0.541 & 0.613 & 255.000 \\
1 & 0.429 & 0.607 & 0.503 & 145.000 \\
accuracy & 0.565 & 0.565 & 0.565 & 0.565 \\
macro avg & 0.568 & 0.574 & 0.558 & 400.000 \\
weighted avg & 0.607 & 0.565 & 0.573 & 400.000 \\
\bottomrule
\end{tabular}

\begin{tabular}{lrr}
\toprule
 & Spearman & Pearson \\
\midrule
0 & 0.244 & 0.241 \\
\bottomrule
\end{tabular}


\subsubsection{Using Summary story and Reasoning text}
\paragraph{Dev}
\begin{tabular}{lrrrr}
\toprule
 & precision & recall & f1-score & support \\
\midrule
0 & 0.830 & 0.629 & 0.716 & 62.000 \\
1 & 0.566 & 0.789 & 0.659 & 38.000 \\
accuracy & 0.690 & 0.690 & 0.690 & 0.690 \\
macro avg & 0.698 & 0.709 & 0.687 & 100.000 \\
weighted avg & 0.730 & 0.690 & 0.694 & 100.000 \\
\bottomrule
\end{tabular}

==> Assets/extra.tex <==
The challenge of operationalizing empathic similarity involves creating a framework that can accurately capture and analyze the nuanced emotional landscapes of personal narratives. The task is formulated around the goal of retrieving and analyzing stories that are not just thematically similar but resonate on a deeper emotional level. By employing a model that evaluates stories based on a composite similarity score—encompassing the main event, emotional reaction, and moral—the researchers aim to discern stories that mirror one another in the empathic essence they convey.

This approach requires developing sophisticated AI models that can go beyond surface-level textual analysis to understand the emotional and moral underpinnings of narratives. The use of fine-tuned large language models (LLMs) and bi-encoder architectures represents a significant advancement in this direction, enabling the efficient retrieval of empathically similar stories while capturing the complexity of human emotions.



\subsection{Recent Observation} 
Recent paper \cite{Jang2023ExploringTB} suggests that the expert language training model (LM) instead of Instruction Tuning has advantages for some cases. For this stream, we need to consider model similar to \cite{Li2020EmpDGMI}. 

\subsection{2nd Observation} To enhance empathy in Large Language Models (LLMs), it is crucial to reassess the specific task we are focusing on. Several notable papers, which I'll reference shortly, have tried to address this objective by refining responses to exhibit more empathetic behavior. These approaches aligns more closely with the goal (enhancing empathy in LLMs) compared to the task we're currently exploring. Even our target is not just enhancing the empathy in LLMs but also to leverage this \cite{shen-etal-2023-modeling} new benchmark, still I believe this empathical rich response generator models can serve as feature extractor and we can finetune them to generalize for similarity classification. 


\citet{Rashkin2018TowardsEO} suggested that models trained on their released \textbf{EmpathicDialogue} benchmark could enhance empathy in dialogue systems. Similarly, \cite{Majumder2020MIMEME} introduced the concept of mimicking user emotions to varying extents, based on the emotional tone and context, to improve both empathy and contextual relevance in responses. Building on these insights, Li et al. \cite{Li2020EmpDGMI} emphasized the importance of fine-grained emotional analysis, arguing that understanding dialogue-level emotion requires attention to word-level emotional cues. They labeled emotional words in the EmpathicDialogue using an external emotion lexicon \cite{mohammad2013crowdsourcing}, leading to significant improvements. Sabour et al. \cite{Sabour2021CEMCE} enhanced empathy in dialogue by incorporating commonsense knowledge and user situations, utilizing the ATOMIC \cite{sap2019atomic} knowledge base for generating commonsense inferences.



% \begin{table*}[]

%     \centering
%     \resizebox{\textwidth}{!}{
%     \begin{tabular}{l|c|c|ccccc}
%     \hline
%         \textbf{Label\_score} & \textbf{Model} & \textbf{Loss} & \textbf{Accuracy} & \textbf{Macro\_F1} & \textbf{Weighted\_F1} & \textbf{$r$} & \textbf{$\rho$} \\ \hline
%         Event & multi-qa & Contrastive & 0.625 & 0.6241 & 0.6236 & \textbf{0.3707} & \textbf{0.3648 }\\ 
%         Event & roberta-base & Contrastive & \textbf{0.635} & \textbf{0.6346} & \textbf{0.6342} & 0.3180 & 0.3087 \\ \hline
        
%         Emotion & roberta-base & CosineSimilarity & 0.\textbf{6525} & 0.\textbf{6501} & \textbf{0.6508} & 0.3775 & 0.3715 \\ 
%         Emotion & roberta-large & CosineSimilarity & 0.62 & 0.6112 & 0.6127 & \textbf{0.3936} & \textbf{0.3880} \\ \hline
        
%         %Moral & roberta-large & CoSENT & 0.65 & 0.6499 & 0.6499 & 0.2875 & 0.3114 \\ 
%         Moral & roberta-base & AnglE & \textbf{0.65} & \textbf{0.6499} & \textbf{0.6501} & 0.3262 & 0.3236 \\ 
%         Moral & multi-qa & CosineSimilarity & 0.6075 & 0.6045 & 0.6036 & \textbf{0.3871} & \textbf{0.3744} \\ \hline
        
%         Empathy & roberta-base & CosineSimilarity & 0.62 & 0.6087 & 0.6104 & \textbf{0.4042} & 0.3886 \\ 
%         Empathy & multi-qa & CosineSimilarity & \textbf{0.6475} & \textbf{0.6475} & \textbf{0.6475} & 0.3999 & \textbf{0.3957} \\ \hline
%     \end{tabular}
%     }
% \caption{Results of Language Models, Fine-tuned on annotation score of key story features \textbf{event}, \textbf{emotion} and \textbf{moral} \& overall \textbf{empathy} score }
%     \label{tab:lm-finetuning}
% \end{table*}

\begin{table*}[t!]
\small
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{lllllll}
\toprule
\textbf{Model} & \textbf{Gold label} & \textbf{Accuracy} & \textbf{Macro\_F1} & \textbf{Weighted\_F1} & \textbf{Pearson} & \textbf{Spearman} \\ 
\midrule
\textbf{event} & \textbf{multi-qa-MiniLM-L6-cos-v1} & \textbf{0.74}     & \textbf{0.6148}    & \textbf{0.7323}       & \textbf{0.3116}  & \textbf{0.2945}   \\ 
emotion        & multi-qa-MiniLM-L6-cos-v1          & 0.56              & 0.5005             & 0.5152                & 0.2262           & 0.226             \\ 
moral          & multi-qa-MiniLM-L6-cos-v1          & 0.61              & 0.5334             & 0.5722                & 0.2166           & 0.2144            \\ 
empathy        & multi-qa-MiniLM-L6-cos-v1          & 0.55              & 0.5086             & 0.5051                & 0.2209           & 0.2136            \\ \hline
event          & multi-qa-mpnet-base-dot-v1         & 0.315             & 0.3032             & 0.2547                &\textbf{0.3684}          & \textbf{0.3478}          \\ 
emotion        & multi-qa-mpnet-base-dot-v1         & \textbf{0.515} & \textbf{0.445}  & \textbf{0.4283}              & 0.3182           & 0.2976            \\ 
moral          & multi-qa-mpnet-base-dot-v1         & 0.445             & 0.392              & 0.3553                & 0.2744           & 0.256             \\
empathy        & multi-qa-mpnet-base-dot-v1         & 0.54              & 0.447              & 0.4527                & 0.2635           & 0.23895           \\ \hline
\end{tabular}
}
\caption{\textbf{Cosine similarity($v_a$, $v_b$) across three sentence embedding models} evaluation results on test set over four type of gold similarity scores: \textbf{event}, \textbf{emotion}, \textbf{moral} \& and \textbf{empathy}.}
    \label{tab:lm-unsupervise}
\end{table*}


















\begin{table*}[]
\begin{tabular}{lllrrrrrr}
\hline
label   & model       & loss                 & \multicolumn{1}{l}{P} & \multicolumn{1}{l}{S} & \multicolumn{1}{l}{Acc} & \multicolumn{1}{l}{Prec} & \multicolumn{1}{l}{Recall} & \multicolumn{1}{l}{F1-Macro} \\ \hline
emotion & robertbase  & CosineSimilarity & 0.3775                      & 0.3715                       & 0.6525                       & 0.6538                   & 0.6508                     & 0.6501                        \\ \hline
emotion & robertlarge & CosineSimilarity & 0.3936                      & 0.3880                       & 0.6200                       & 0.6261                   & 0.6166                     & 0.6113                        \\ \hline

moral   & robertbase  & AnglELoss            & 0.3262                      & 0.3236                       & 0.6500                       & 0.6499                   & 0.6500                     & 0.6499                        \\ \hline
moral   & MPNET    & CosineSimilarity & 0.3871                      & 0.3744                       & 0.6075                       & 0.6146                   & 0.6101                     & 0.6045                        \\ \hline
event   & MPNET    & Contrastive      & 0.3707                      & 0.3648                       & 0.6250                       & 0.6286                   & 0.6266                     & 0.6241                        \\ \hline
event   & robertbase  & ContrastiveLoss      & 0.3180                      & 0.3087                       & 0.6350                       & 0.6374                   & 0.6363                     & 0.6346                        \\ \hline
empathy & robertbase  & CosineSimilarity & 0.4042                      & 0.3886                       & 0.6200                       & 0.6288                   & 0.6161                     & 0.6087                        \\ \hline
empathy & MPNet    & CosineSimilarity & 0.3999                      & 0.3957                       & 0.6475                       & 0.6476                   & 0.6477                     & 0.6475                        \\ \hline
\end{tabular}
\caption{Results of Language Models, fine-tuned on annotation score of key story features \textbf{event}, \textbf{emotion} and \textbf{moral} \& overall \textbf{empathy} score }
    \label{tab:lm-finetuning}
\end{table*}




\begin{table*}[t!]
    \centering
    \resizebox{\textwidth}{!}{
    \begin{tabular}{@{}lcccccccccccccc@{}}
    \toprule
    \multicolumn{1}{l|}{\textbf{Testbed$\rightarrow$}} & \multicolumn{7}{c|}{\textbf{Development Set}} & \multicolumn{7}{c}{\textbf{Test Set}} \\
    \multicolumn{1}{l|}{\textbf{Gold Label$\downarrow$}} & \textbf{$r$} & \textbf{$\rho$} & \textbf{MSE}$\downarrow$ & \textbf{Acc} & \textbf{Prec} & \textbf{Recall} & \multicolumn{1}{c|}{\textbf{F1-macro}} & \textbf{$r$} & \textbf{$\rho$} & \textbf{MSE}$\downarrow$ & \textbf{Acc} & \textbf{Prec} & \textbf{Recall} & \textbf{F1-macro} \\ \midrule
    \multicolumn{15}{c}{\texttt{OpenAI-text-embedding-3-large} (Summary)} \\ 
    \midrule
    \multicolumn{1}{l|}{\textbf{Empathy}} & 0.335 & 0.315 & 1.280 & 0.630 & 0.813 & 0.513 & 0.411 
    & \multicolumn{1}{|l}{0.336} & 0.329 & 1.510 & 0.505 & 0.633 & 0.517 & 0.376 \\
    \multicolumn{1}{l|}{\textbf{Event}} & 0.437 & 0.411 & 0.600 & 0.820 & 0.414 & 0.494 & 0.451 
    & \multicolumn{1}{|l}{0.485} & 0.465 & 0.620 & 0.780 & 0.738 & 0.542 & 0.522 \\
    \multicolumn{1}{l|}{\textbf{Emotion}} & 0.394 & 0.350 & 1.130 & 0.720 & 0.859 & 0.517 & 0.451 
    & \multicolumn{1}{|l}{0.392} & 0.388 & 1.310 & 0.550 & 0.582 & 0.510 & 0.392 \\
    \multicolumn{1}{l|}{\textbf{Moral}} & 0.359 & 0.309 & 0.960 & 0.800 & 0.899 & 0.524 & 0.489 
    & \multicolumn{1}{|l}{0.366} & 0.356 & 1.210 & 0.620 & 0.692 & 0.525 & 0.437 \\
    \midrule
    \multicolumn{15}{c}{\texttt{OpenAI-text-embedding-3-large} (Full)} \\ 
    \midrule
    \multicolumn{1}{l|}{\textbf{Empathy}} & 0.303 & 0.309 & 1.400 & 0.620 & 0.561 & 0.505 & 0.406
    & \multicolumn{1}{|l}{0.362} & 0.363 & 1.440 & 0.507 & 0.624 & 0.519 & 0.384 \\
    \multicolumn{1}{l|}{\textbf{Event}} & 0.385 & 0.409 & 0.680 & 0.810 & 0.413 & 0.488 & 0.448
    & \multicolumn{1}{|l}{0.488} & 0.469 & 0.590 & 0.782 & 0.737 & 0.551 & 0.538 \\
    \multicolumn{1}{l|}{\textbf{Emotion}} & 0.345 & 0.361 & 1.260 & 0.710 & 0.607 & 0.510 & 0.446 
    & \multicolumn{1}{|l}{0.393} & 0.386 & 1.260 & 0.568 & 0.685 & 0.529 & 0.421 \\
    \multicolumn{1}{l|}{\textbf{Moral}} & 0.337 & 0.325 & 1.050 & 0.790 & 0.648 & 0.517 & 0.484 
    & \multicolumn{1}{|l}{0.395} & 0.403 & 1.140 & 0.618 & 0.651 & 0.524 & 0.440 \\

    \bottomrule
    \end{tabular}%
    }
    \caption{\textbf{Cosine similarity($v_a$, $v_b$) across three sentence embedding models.} Results on dev and test sets over four type of gold similarity scores: \textbf{empathy}, \textbf{event}, \textbf{emotion} and \textbf{moral} based on full story or summary. Cosine similarity is normalized to the scale 1-4 by $\times$4. Classification gold labels are binned by $\text{score} > 2.5$.}
    \label{tab:lm-unsupervise-cosine}
    % \vspace{-1em}
\end{table*}

==> section/tabels/ft_dis_model_perf.tex <==

\begin{table}[ht!]
    \centering
    % \resizebox{0.7\textwidth}{!}{
    \resizebox{\columnwidth}{!}{
    \begin{tabular}{@{}l|l|l|cc|cccc@{}}
    \toprule
    %\multicolumn{8}{c}{\textbf{Test Set}} \\
    \multicolumn{1}{l|}{\textbf{Train Label$\downarrow$}} & \textbf{Model} & \multicolumn{1}{l|}{\textbf{Loss}} & 
    %\textbf{$r$} & \textbf{$\rho$} & \textbf{Acc} & \textbf{Prec} & \textbf{Recall} & \multicolumn{1}{c|}{\textbf{F1-macro}} 
    \textbf{$r$} & \textbf{$\rho$}  & \textbf{Acc} & \textbf{Prec} & \textbf{Recall} & \textbf{F1-macro} \\ 
    \midrule
     \multicolumn{9}{c}{\texttt{\empathicstories Baselines} (Summary)} \\ 
    \midrule
    \textbf{Empathy} & SBERT & MSE & 0.359 & 0.352 & 0.648 & 0.587 & 0.907 & 0.713 \\
    \textbf{Empathy} & BART & MSE & 0.342 & 0.344 & 0.648 & 0.582 & 0.883 & 0.701 \\
    \textbf{Empathy} & GPT-3.5-turbo & NA/5-shot & 0.278 & 0.281 & 0.633 & 0.604 & 0.820 & 0.696 \\
    \midrule
    \multicolumn{9}{c}{\texttt{Contrastive Loss of LMs} (Summary)} \\
    \midrule
    \textbf{Empathy} & RoBerta-base & Cosine & \textbf{0.404} &	0.388 &	0.620	& 0.628 &	0.616 &	0.608 \\
    \textbf{Empathy} & Multi-qa-MPNet & Cosine  & 0.400	& \textbf{0.395} & 0.647 &	0.647	& 0.647 & 0.647 \\ 
    \midrule
    \textbf{Event} & RoBerta-base & Contrastive & 0.318	& 0.3087	& 0.635 &	0.637 & 0.636 & 0.634 \\
    \textbf{Event} & Multi-qa-MPNet & Contrastive &  0.370	& 0.364	& 0.625 &	0.628 &	0.626 &	0.624 \\
    \midrule
    \textbf{Emotion} & RoBerta-base & Cosine & 0.377	& 0.371	& \textbf{0.652} &	\textbf{0.653} &	\textbf{0.650} & \textbf{0.650} \\
    \textbf{Emotion} & RoBerta-large & Cosine & 0.393 & 0.388 &	0.620 &	0.626 &	0.616 &	0.611 \\ 
    \midrule
    \textbf{Moral} & RoBerta-base & AnglELoss & 0.326 &	0.323 &	0.650 &	0.649 & \textbf{0.650} &	0.649 \\
    \textbf{Moral} & Multi-qa-MPNet & Cosine & 0.387 &	0.374	& 0.607 &	0.614 &	0.610	& 0.604 \\
    % \multicolumn{1}{l|}{\textbf{}} & \multicolumn{1}{l|}{\text{}} & \multicolumn{1}{l|}{\text{}}  & \textbf{0.404} &	0.388 &	0.620	& 0.628 &	0.616 &	0.608 \\
    % \multicolumn{1}{l|}{\textbf{Empathy}} & \multicolumn{1}{l|}{\text{Multi-qa-MPNet}} & \multicolumn{1}{l|}{\text{Cosine}} & 0.400	& \textbf{0.395}	& \textbf{0.647} &	\textbf{0.647}	& \textbf{0.647}	& \textbf{0.647} \\ \midrule
    % \multicolumn{1}{l|}{\textbf{Event}} & \multicolumn{1}{l|}{\text{RoBerta-base}} & \multicolumn{1}{l|}{\text{Contrastive}}  & 0.318	& 0.3087	& \textbf{0.635} &	\textbf{0.637} &	\textbf{0.636} &	\textbf{0.634} \\
    % \multicolumn{1}{l|}{\textbf{Event}} & \multicolumn{1}{l|}{\text{Multi-qa-MPNet}} & \multicolumn{1}{l|}{\text{Contrastive}} &  \textbf{0.370}	& \textbf{0.364}	& 0.625 &	0.628 &	0.626 &	0.624 \\
    % \midrule
    %\multicolumn{15}{c}{\texttt{OpenAI-text-embedding-3-large} (Full)} \\ 
    %\midrule
    % \multicolumn{1}{l|}{\textbf{Emotion}} & \multicolumn{1}{l|}{\text{RoBerta-base}} & \multicolumn{1}{l|}{\text{Cosine}} & 0.377	& 0.371	& \textbf{0.652} &	\textbf{0.653} &	\textbf{0.650} &	\textbf{0.650} \\
    % \multicolumn{1}{l|}{\textbf{Emotion}} & \multicolumn{1}{l|}{\text{RoBerta-large}} & \multicolumn{1}{l|}{\text{Cosine}} & \textbf{0.393} &	\textbf{0.388} &	0.620 &	0.626 &	0.616 &	0.611 \\ \midrule
    % \multicolumn{1}{l|}{\textbf{Moral}} & \multicolumn{1}{l|}{\text{RoBerta-base}} & \multicolumn{1}{l|}{\text{AnglELoss}}  & 0.326 &	0.323 &	\textbf{0.650} &	\textbf{0.649} &	\textbf{0.650} &	\textbf{0.649} \\
    % \multicolumn{1}{l|}{\textbf{Moral}} & \multicolumn{1}{l|}{\text{Multi-qa-MPNet}} & \multicolumn{1}{l|}{\text{Cosine}} & \textbf{0.387} &	\textbf{0.374}	& 0.607 &	0.614 &	0.610	& 0.604 \\
    \bottomrule
    \end{tabular}%
    }
\caption{Test set results of LMs fine-tuned over annotations of \textbf{event}, \textbf{emotion}, \textbf{moral} and the overall \textbf{empathy} score and tested on \textbf{empathy} vs. baseline results obtained from \citet{shen-etal-2023-modeling}.}
    \label{tab:lm-finetuning}
    % \vspace{-1em}
\end{table}


